Software Engineering For Automated Game Design

As we develop more assistive and automated game design systems, the question of how these systems should be integrated into game development workflows, and how much adaptation may be required, becomes increasingly important. In this paper we explore the impact of software engineering decisions on the ability of an automated game design system to understand a game's codebase, generate new game code, and evaluate its work. We argue that a new approach to software engineering may be required in order for game developers to fully benefit from automated game designers.

==> README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/

For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


***************************** Subdirectories ******************************

bibtex   - The IEEEtran BibTeX style package.

extras   - Supplementary material that may be of interest.

testflow - The testflow diagnostic suite for verifying PS/PDF output.

tools    - The IEEEtrantools.sty package which provides several commands
           from the IEEEtran.cls file for use with other LaTeX classes.


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf.tex          - A bare bones starter file for IEEE conference papers.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl.tex          - A bare bones starter file for IEEE journal papers.

bare_jrnl_comsoc.tex   - A bare bones starter file for IEEE Communications
                         Society journal papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_jrnl_transmag.tex - A bare bones starter file for IEEE Transactions
                         on Magnetics journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for an IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf.tex, bare_conf_compsoc.tex,
                   bare_jrnl.tex, bare_jrnl_comsoc.tex,
                   bare_jrnl_compsoc.tex, bare_jrnl_transmag.tex
***************************************************************************


==> trash.tex <==


\section{Reflection-Driven Automated Game Design}
\textbf{TODO: A high-level description of the code generation system.}

We have envisaged a system which is initially configured and set up through a collaboration between designers and programmers, but can then be used easily by designers with minimal code editing. In this section we provide an overview of the system's structure,

The emphasis of our framework is simplicity of installation, use and interpretation of results. Our system is easily integrated into a new game's codebase, with some simple configuration work to adjust the scope of its design space. The system can then be given a testing environment,

The emphasis of our framework is on simplicity of installation, use and interpretation of results. Our system generates code blocks which are designed to be placed in specific parts of the


\section{Reflection-Driven Automated Game Design}
In this section we describe a framework for automated game design systems that integrates directly into common game development practice. The automated game designer works at the level of code, rather than using a higher-level abstract representation such as a GDL. Interactions with the designer are also done through code -- shaping and configuring it by adding metadata to the codebase, and then invoking its design capabilities through API calls. We believe that a framework such as this would be more easily adopted by the majority of game developers, as it fits into the way games are currently developed (and have been developed for decades). We discuss the nature of change in development practices in section \ref{sec:discussion}. %While, of course, we cannot assume the future will not bring changes, it is also undeniably the case that practices change extremely slowly

\subsection{System Description}
Our systems is implemented within Unity, using the C\# programming language. The system does not use any Unity-specific features, however, and would work on any C\# codebase, and the approach as a whole uses fairly common language features that could be ported easily to most modern programming languages.

The main function of the system is to generate code blocks, matching a specification which constraints some features of the generated code. Primarily these code blocks are used as method bodies, and the specification is used to specify the method's type signature (fixing the local scope of the code block, i.e. the arguments to the method, and the return type the method must have if applicable). These code blocks can be compiled at runtime and stored in objects called \textit{delegates}, which are objects that represent methods with a particular method signature. They can be stored as variables, passed around as data, and invoked like methods. Listing \ref{lst:delegates} shows an example of a delegate type being declared, then used to create a delegate object, and that object being invoked.


\begin{figure}
\begin{lstlisting}
//Declares a new type of delegate, NumberOp
public delegate int NumberOp(int x);

//Declares a variable of type NumberOp
public NumberOp numDelegate;

public int AddOne(int x){ return x + 1; }

public void Start(){
    //Assigns the method AddOne to the
    //delegate numDelegate
    numDelegate = new NumberOp(AddOne);
    //This prints "2"
    Print(changeNumber(1));
}
\end{lstlisting}
\caption{A code snippet showing delegate usage.}
\label{lst:delegates}
\end{figure}

\begin{figure}
\begin{lstlisting}
public delegate void ButtonPress();
public ButtonPress onActionButton = DoNothing;

public void DoNothing(){}

public void Update(){
    if(Input.GetKeyDown(KeyCode.X)){
        onActionButton();
    }
}
\end{lstlisting}
\caption{A code snippet showing a delegate called in response to player input. The button's default assignment is a void method DoNothing, which avoids a possible null reference if the delegate is not assigned.}
\label{lst:delegates}
\end{figure}

As an illustration of how this system fits into an existing codebase, consider a grid-based puzzle game played on a grid of coloured tiles. When a tile is tapped, the code invokes a method called \verb|OnTileTapped| which handles the game logic for interacting with a tile. In our system, this method call is replaced with the invocation of a delegate which has the same type signature as \verb|OnTileTapped|. By default, this will run the game's regular logic, which might be to destroy the tile and have other tiles above it fall down. However, if a designer wishes to explore alternate mechanics for tapping on tiles, our system can be asked to generate a code block to replace this existing logic, and swap its generated delegate in for the game's normal code. Editing the code to allow for this requires adding just three lines of code, as well as editing one existing line. By doing so, our system can now dynamically swap in code to replace this piece of functionality.

\subsection{Generating Code Snippets}
We represent a code block as a list of lists of strings. Each list of strings represents a single line of code, which is built up incrementally. For this prototype system we work with a restricted subset of the C\# language; each line may be one of the following statement types: an assignment, a variable declaration, a method invocation or an if/else statement.

Any time an expression of a particular type is needed, the code generator will search all available scopes for any object that fulfils this type. This includes: any \textbf{static} or \textbf{non-static} methods in scope with a matching return type; any \textbf{static} or \textbf{non-static} fields or \textbf{local} variables of a matching type; and a \textbf{literal expression} of that type (where applicable). All possible expressions are chosen from with equal weight, with the exception of literal expressions whose weight can be adjusted but is treated as a single `option'. The reason for this is that the number of possible literal expressions may be very large -- in the case of an integer type expression with no constraints, there are $2^{64}$ possible values, and so it is easier to treat the literal expression as a single option with a set weight, and then if it is chosen simple pick uniformly from any valid literal value.

The reader will note that the local scope is dynamic -- the declaration of new variables adds new elements to the scope, as that variable may be used in code lines added afterwards. A code block is always generated in execution sequence for this reason. Note also that generating an expression of a certain type may result in recursive searches for more expressions: for example, if we generate a method invocation, and that method has arguments, we will need to generate an expression for each of these arguments too. To avoid a situation in which this recursion continues indefinitely, we limit the number of times the expression generation can recurse. Once it has reached this limit, we will only generate grounded expressions, i.e. no parameterised method calls.



%Our system generates blocks of code which conform to a specification that includes a description of the scope at the beginning of the code block. The specification may also require that the code block returns a value of a particular type. Typically, these code blocks are intended to be the body of a method -- the scope describes the arguments to the method, and the return type (if present in the specification) describes the method's return type. In our target language, C\#, these code blocks can be compiled at runtime and executed dynamically using \textit{delegates}, a C\# type that defines a reference to a method with a particular type signature. Delegates allow for code to be dynamically altered at runtime by replacing method calls with calls to different methods that share the same type signature.
%
%Thus, consider a puzzle game played on a grid of coloured tiles. When a tile is tapped, a method, \verb|OnTapTile|, is called. Our automated game design system can generate a method with the same type signature as \verb|OnTapTile| and replace it at runtime. This can be done as part of a closed loop to try and generate and evaluate new code, or as part of an interactive mode where a designer or other used plays the game with the generated code swapped in.
%

\subsection{Narrowing Generative Scope With Annotations}
In the previous section we described how the system searches to find possible expressions that match a specific type. If it were to do this across the entire game's codebase the search would be far too extensive, creating a very large possibility space that is hard to search. Additionally, even if such large-scale a search could be made tractable, code generated using all fields and methods in a game's codebase could potentially have side effects that persist outside of an execution of the game (for example, calling methods that erase save games or reset preferences).

We also wish to provide ways for a designer or programmer to interact with the system and express their own intentions, ideas and focus. For example, if they are interested in designing a new way for the player to solve problems without killing characters, they might wish to stop the AGD system from using parts of the codebase related to fighting or dealing damage.

To achieve this, we propose the use of \textit{annotations}, allowing the user both to reduce the complexity of the search problem the AGD system is solving, as well as allowing them to direct the focus of the system onto parts of the game they are interested in working with.

An \textit{annotation} is a marker that can be used to label a section of code in the C\# language. This marker can be detected at runtime through reflection, which allows a program to retrieve parts of a codebase labelled by a user. In our past projects we have used annotations to allow the user to label parts of a procedural generator they wanted to analyse using a tool, for example \cite{danesh}.

\begin{figure}
\begin{lstlisting}
[Usable]
public int x;

[Usable("newx", "min", -1, "newx", "max", 1)]
public void Move(int newx){
    //...
}
\end{lstlisting}
\caption{A field and method annotated with a Usable annotation. The method's annotation provides contextual information about the parameter \texttt{newx}.}
\label{lst:annotation}
\end{figure}

In our system we introduce an annotation called \texttt{Usable}. This annotation is attached to methods and parameters by a user, which then makes the parameter or method part of the design space available to the automated game designer at runtime. When generating code, our AGD system searches only for methods and fields with the \texttt{Usable} annotation, and does not include any other code in its search space (other than variables directly in scope, such as method arguments). Listing \ref{lst:annotation} shows an example where a field \texttt{x} has been labelled with the \texttt{Usable} annotation.

Listing \ref{lst:annotation} also shows a parameterised version of the \texttt{Usable} annotation. Annotations can be constructed with data which can be retrieved through reflection as well. Our system supports the specification of simple constraints through a list of objects, by supplying the name of a parameter, the type of constraint (currently either minimum value or maximum value) and then an object which completes the constraint and is the same type as the parameter (e.g. an integer if the constraint affects an integer parameter).

